MOY calculus in type D

We define a positive state sum for webs "of type D". These webs are graphs which mimic morphisms in the category of finite-dimensional quantum so(2N)-modules. From the state sum, we derive an invariant of framed unoriented links. After giving explicit details about some intertwiners in the category of quantum so(2N)-modules, we relate our state-sum link invariant with Reshetikhin--Turaev's invariant associated with quantum so(2N).

==> td-PF-macros.tex <==
\newcommand{\ccc}[1]{
  \begin{scope}[xscale=#1]
  \foreach \i in {18, 90, 162, 234, 306}{
    \coordinate (A\i) at (\i:1);
    \coordinate (a\i) at (\i:0.8);
  }
  \coordinate (b90) at (270:-0.3);
  \coordinate (b270) at (270:0.3);
    \coordinate (s) at (-0.1,0);
  \begin{scope}[shift = {(-0.45, -0.077)}, rotate=15]
    \coordinate (l0) at (0,0);
    \foreach \j in {90, 180, 270, 360}{
      \coordinate (l\j) at (\j:0.21);}
  \end{scope}    
  \end{scope}
  }
  \newcommand{\smootha}[2]{
  \draw[expand style= \stylevect] (A162) .. controls (a162) .. (l90);
  \draw[expand style= \stylevect] (b270) .. controls + (s) .. (l270);
  \draw[expand style= #1] (b90) -- (l90) \arr;
  \draw[expand style= #1] (A234) .. controls (a234) .. (l270) \arr ;
  \draw[expand style= #2] (l90) -- (l270) \rarr;
  }
\newcommand{\smoothb}[2]{
    \draw[expand style= \stylevect] (A162) .. controls (a162) .. (l180);
  \draw[expand style= \stylevect] (b270) .. controls + (s) .. (l360);
  \draw[expand style= #1] (b90) -- (l360) \arr;
  \draw[expand style= #1] (A234) .. controls (a234) .. (l180) \rarr ;
  \draw[expand style= #2] (l180) -- (l360) \arr;
}
\newcommand{\ddd}[3][]{\NB{\tikz[#1]{
\begin{scope}
  \ccc{1}
  \draw[expand style= \stylevect] (A90) -- (b90);
  #2{\styleeven}{\styleodd}
  \ccc{-1}
  #3{\styleodd}{\styleeven}
\end{scope}}}}


% \begin{scope}
%   \foreach \i in {18, 90, 162, 234, 306}{
%     \coordinate (A\i) at (\i:1);
%     \coordinate (a\i) at (\i:0.85);
%   }
%   \coordinate (b90) at (270:-0.3);
%   \coordinate (b270) at (270:0.3);

%   \coordinate (s) at (-0.1,0);
%   \begin{scope}[shift = {(-0.45, -0.077)}, rotate=15]
%     \coordinate (l0) at (0,0);
%     \foreach \j in {90, 180, 270, 360}{
%       \coordinate (l\j) at (\j:0.21);}
%     \foreach \j in {45, 135, 225, 315}{
%       \coordinate (K\j) at (\j:0.2);}
%   \end{scope}
  




%   \draw[expand style= \styleodd] (b90) .. controls (a18) and (a306) .. (A306) \arrodd coordinate[pos=0.275] (x);

%   \draw[expand style= \stylevect] (A90) -- (b90);%  coordinate[pos=0.6482] (x);
  
  
% \end{scope}
% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: t
% %%% End:


==> td-R2-macros.tex <==
\newcommand{\ccc}{
  \coordinate (o) at (0.5,0.5);
  \coordinate (a) at (0,1);
  \coordinate (b) at (1,1);
  \coordinate (c) at (1,0);
  \coordinate (d) at (0,0);
}

\newcommand{\dd}[2][]{
      \NB{\tikz[#1]{
      \begin{scope}[expand style = \stylevect]
        \begin{scope}[xscale=2]
          \ccc
        \end{scope}
        #2
        \end{scope}}}}
        
\newcommand{\ddd}[3][]{
  \NB{\tikz[#1]{
      \begin{scope}[expand style = \stylevect]
      \ccc
      #2
    \begin{scope}[xshift =1cm]
      \ccc
      #3
    \end{scope}
  \end{scope}}}}

\newcommand{\xing}{
  \draw (a) .. controls +(0.3, 0) and +(-0.3, 0) ..  (c);
  \fill[white] (o) circle (1mm);
  \draw (d) .. controls +(0.3, 0) and +(-0.3, 0) .. (b);
}

\newcommand{\xingm}{
  \draw (d) .. controls +(0.3, 0) and +(-0.3, 0) .. (b);
  \fill[white] (o) circle (1mm);
  \draw (a) .. controls +(0.3, 0) and +(-0.3, 0) .. (c);
}
\newcommand{\sing}{
  \draw (d) .. controls +(0.3, 0) and +(-0.3, 0) .. (b);
  \node at (o) {\singvertex};
  \draw (a) .. controls +(0.3, 0) and +(-0.3, 0) .. (c);
}
\newcommand{\horz}{
  \draw (a) -- (b);
  \draw (d) -- (c);
}
\newcommand{\vertz}{
  \draw (c) .. controls +(-0.3, 0) and +(-0.3, 0) .. (b);
  \draw (a) .. controls +(0.3, 0) and +(0.3, 0) .. (d);
}




==> td-R2sv-macros.tex <==
\newcommand{\ccc}[1]{
%\coordinate (smr) at (0.1,0);
  \begin{scope}[xscale=#1]
  \coordinate (A) at (-1, 0.5);
  \coordinate (B) at (0, 0.5);
  \coordinate (C) at (0, -0.5);
  \coordinate (D) at (-1, -0.5);
  \coordinate (O) at (-0.5, 0);
  \coordinate (t) at (-0.5,0.25);
  \coordinate (b) at (-0.5,-0.25);
  \coordinate (l) at (-0.75,0);
  \coordinate (r) at (-0.25,0);
  \coordinate (sl) at (-0.25,0);
  \coordinate (sr) at ( 0.25,0);
\end{scope}}

\newcommand{\unknotted}[2]{
\begin{scope} 
  \draw[expand style = #1] (A) -- (B) \arr;
  \draw[expand style = \stylevect] (D) -- (C);
\end{scope}}

\newcommand{\xing}[2]{
\begin{scope}
  \draw[expand style = #1] (A) .. controls +(sr) and +(0,0) .. (O) \arr  .. controls +(0,0) and +(sl) .. (C) \arr;
  \fill[white] (O) circle (1mm);
  \draw[expand style =\stylevect] (D) .. controls +(sr) and +(sl) .. (B);
\end{scope}}

\newcommand{\xingm}[2]{
  \begin{scope}
  \draw[expand style =\stylevect] (D) .. controls +(sr) and +(sl) .. (B);
  \fill[white] (O) circle (1mm);
  \draw[expand style = #1] (A) .. controls +(sr) and +(sl) .. (C) \arr ;
\end{scope}
}

\newcommand{\III}[3][\rarr]{
\begin{scope}
  \draw[expand style = #2] (A) .. controls +(sr) and +(0,0) .. (t) \arr;
  \draw[expand style = #2] (C) .. controls +(sl) and +(0,0) .. (b) \arr;
  \draw[expand style = \stylevect] (D) .. controls +(sr) and +(0,0) .. (b) ;
  \draw[expand style = \stylevect] (B) .. controls +(sl) and +(0,0) .. (t) ;
  \draw[expand style = #3] (b) -- (t) #1;
\end{scope}}

\newcommand{\IIIr}[2]{\III[\arr]{#1}{#2}}

\newcommand{\HHH}[2]{
\begin{scope}
  \draw[expand style = #1] (A) .. controls +(sr) and +(0,0) .. (l) \arr;
  \draw[expand style = #1] (C) .. controls +(sl) and +(0,0) .. (r) \arr;
  \draw[expand style = \stylevect] (D) .. controls +(sr) and +(0,0) .. (l) ;
  \draw[expand style = \stylevect] (B) .. controls +(sl) and +(0,0) .. (r) ;
  \draw[expand style = #2] (l) -- (r) \arr;
\end{scope}}

\newcommand{\ddd}[3][]{\NB{\tikz[#1]{
\begin{scope}
  \ccc{1}
  #2{\styleeven}{\styleodd}
  \ccc{-1}
  #3{\styleeven}{\styleodd}
\end{scope}}}}


\newcommand{\dddodd}[3][]{\NB{\tikz[#1]{
\begin{scope}
  \ccc{1}
  #2{\styleodd}{\styleodd}
  \ccc{-1}
  #3{\styleodd}{\styleodd}
\end{scope}}}}


\newcommand{\dd}[2][]{\NB{\tikz[#1]{
\begin{scope}
  \ccc{2}
  #2{\styleeven}{\styleodd}
\end{scope}}}}

\newcommand{\ddodd}[2][]{\NB{\tikz[#1]{
\begin{scope}
  \ccc{2}
  #2{\styleodd}{}
\end{scope}}}}





%   \draw[expand style= \styleodd] (b90) .. controls (a18) and (a306) .. (A306) \arrodd coordinate[pos=0.275] (x);

%   \draw[expand style= \stylevect] (A90) -- (b90);%  coordinate[pos=0.6482] (x);
  
  
% \end{scope}
% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: t
% %%% End:

